Open-Domain Safety Policy Construction

Moderation layers are increasingly a core component of many products built on user- or model-generated content. However, drafting and maintaining domain-specific safety policies remains costly. We present Deep Policy Research (DPR), a minimal agentic system that drafts a full content moderation policy based on only human-written seed domain information. DPR uses a single web search tool and lightweight scaffolding to iteratively propose search queries, distill diverse web sources into policy rules, and organize rules into an indexed document. We evaluate DPR on (1) the OpenAI undesired content benchmark across five domains with two compact reader LLMs and (2) an in-house multimodal advertisement moderation benchmark. DPR consistently outperforms definition-only and in-context learning baselines, and in our end-to-end setting it is competitive with expert-written policy sections in several domains. Moreover, under the same seed specification and evaluation protocol, DPR outperforms a general-purpose deep research system, suggesting that a task-specific, structured research loop can be more effective than generic web research for policy drafting. We release our experiment code at https://github.com/xiaowu0162/deep-policy-research.

==> figures/data_examples.tex <==
\clearpage

% Thumbnail sizing (tune once)
\newcommand{\thumbw}{2.7cm}
\newcommand{\thumbh}{2.0cm}


\newcommand{\adimg}[1]{%
  \begin{minipage}[t]{\linewidth}\vspace{0pt}\centering
    \includegraphics[width=\thumbw,height=\thumbh,keepaspectratio]{#1}%
  \end{minipage}%
}

% Text cell wrapper to force top alignment
\newcommand{\adtext}[1]{%
  \begin{minipage}[t]{\linewidth}\vspace{0pt}#1\end{minipage}%
}

\begin{figure*}[ht!]
\small
\centering

\begin{tabularx}{\linewidth}{@{}p{3.1cm} X@{}}
\toprule
\multicolumn{2}{c}{\texttt{Rejected Advertisement Examples}} \\
\midrule

\multicolumn{2}{@{}l@{}}{\textit{Policy Domain: \textcolor{blue}{Exploitative}}} \\[0.6mm]
\adimg{figures/example_figs/1.jpg} & 
\adtext{%
\textbf{Title:} Car Crash in \${city:capitalized}\,? Fight For Compensation!\\
\textbf{Description:} Injured in a Car Accident? Find Car Accident Lawyers in Your Area for Free.\\
\textbf{Human reject reason:} Violent content is prohibited.} \\[1.0mm]

\adimg{figures/example_figs/2.jpg} &
\adtext{%
\textbf{Title:} Hemophilia: Scared? Why Knowledge Is Your Ally\\
\textbf{Description:} Feeling anxious about hemophilia can often stem from not knowing enough about the condition. This guide encourages you to embrace knowledge as a tool for empowerment, showing how understanding hemophilia can transform fear into strength.\\
\textbf{Human reject reason:} Assuming the user already suffers from the disease.} \\

\midrule

\multicolumn{2}{@{}l@{}}{\textit{Policy Domain: \textcolor{blue}{Misrepresentation}}} \\[0.6mm]
\adimg{figures/example_figs/3.jpg} &
\adtext{%
\textbf{Title:} Passed: \$1{,}400/mo Subsidy\\
\textbf{Description:} Americans under 65 could get \$1{,}400/month to spend on groceries, bills, and more.\\
\textbf{Human reject reason:} Title used unqualified amount.} \\[1.0mm]

\adimg{figures/example_figs/4.png} &
\adtext{%
\textbf{Title:} California Gov Will Cover The Cost To Install Solar If You Own A Home In These Zip Codes\\
\textbf{Description:} Smart homeowners in California are using a tax incentivized solar program and other incentives to go solar.\\
\textbf{Human reject reason:} No depiction of court room or flag in the background.} \\

\midrule

\multicolumn{2}{@{}l@{}}{\textit{Policy Domain: \textcolor{blue}{Offensive}}} \\[0.6mm]
\adimg{figures/example_figs/5.png} &
\adtext{%
\textbf{Title:} Top Motorcycle Injury Lawyers: Protect Your Rights Today\\
\textbf{Description:} Discover why hiring a Motorcycle Personal Injury Attorney is crucial. Maximize compensation, reduce stress, and receive expert guidance. Trust us to be your advocate in the pursuit of justice. Contact us today and secure your future.\\
\textbf{Human reject reason:} Violent or shocking imagery.} \\

\midrule

\multicolumn{2}{@{}l@{}}{\textit{Policy Domain: \textcolor{blue}{Problematic\_finance\_claims}}} \\[0.6mm]
\adimg{figures/example_figs/6.jpg} &
\adtext{%
\textbf{Title:} Unbelievable! Earn \$800 a Day from Home?\\
\textbf{Description:} Unlock the ultimate cash flow! Earn \$800 daily from home with our proven method.\\
\textbf{Human reject reason:} Absolute language.} \\

\bottomrule
\end{tabularx}

\caption{Qualitative examples of rejected advertisements across policy domains. Each entry shows the thumbnail (left) and the corresponding title, description, and human rejection reason (right).}
\label{fig:ad_rejection_examples}
\end{figure*}

